Higher-Order, Data-Parallel Structured Deduction

State-of-the-art Datalog engines include expressive features such as ADTs (structured heap values), stratified aggregation and negation, various primitive operations, and the opportunity for further extension using FFIs. Current parallelization approaches for state-of-art Datalogs target shared-memory locking data-structures using conventional multi-threading, or use the map-reduce model for distributed computing. Furthermore, current state-of-art approaches cannot scale to formal systems which pervasively manipulate structured data due to their lack of indexing for structured data stored in the heap. In this paper, we describe a new approach to data-parallel structured deduction that involves a key semantic extension of Datalog to permit first-class facts and higher-order relations via defunctionalization, an implementation approach that enables parallelism uniformly both across sets of disjoint facts and over individual facts with nested structure. We detail a core language, $DL_s$, whose key invariant (subfact closure) ensures that each subfact is materialized as a top-class fact. We extend $DL_s$ to Slog, a fully-featured language whose forms facilitate leveraging subfact closure to rapidly implement expressive, high-performance formal systems. We demonstrate Slog by building a family of control-flow analyses from abstract machines, systematically, along with several implementations of classical type systems (such as STLC and LF). We performed experiments on EC2, Azure, and ALCF's Theta at up to 1000 threads, showing orders-of-magnitude scalability improvements versus competing state-of-art systems.

==> Makefile <==
PACKAGE=icse23
JPACKAGE=toplas

all:  $(PACKAGE).pdf $(JPACKAGE).pdf

%.pdf: %.tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM)  *.pdf *.aux *.log *.out *.bbl *.blg *~* *#*

.PHONY: all docclean clean archive zip


==> aam-table.tex <==
\newcolumntype{C}[1]{>{\centering}m{#1}}
 \begin{table*}
 \centering
\footnotesize
\caption{Control-Flow Analysis Experimental Results: Slog vs. Souffl\'e}\label{tab:results-aam}
 \begin{tabular}{m{.1cm}C{.35cm}C{.5cm}C{.7cm}C{.6cm}cccc | m{.1cm}C{.5cm}C{.75cm}C{.6cm}C{.65cm}cccc}
   \toprule 
 & \multirow{2}{*}{Size}&\multirow{2}{*}{Iters}& \multirow{2}{*}{Cf. Pts}& \multirow{2}{*}{Sto. Sz.}& \multicolumn{2}{c}{$8$ Processes} & \multicolumn{2}{c|}{$64$ Processes} 
 & 
 & \multirow{2}{*}{Size}&\multirow{2}{*}{Iters}& \multirow{2}{*}{Cf. Pts}& \multirow{2}{*}{Sto. Sz.}& \multicolumn{2}{c}{$8$ Processes} & \multicolumn{2}{c}{$64$ Processes} 
\\
 & & & & & \multicolumn{1}{c|}{Slog} & \multicolumn{1}{c||}{Souffl\'e}& \multicolumn{1}{c|}{Slog}& \multicolumn{1}{c|}{Souffl\'e}
 & 
 & & & & & \multicolumn{1}{c|}{Slog} & \multicolumn{1}{c||}{Souffl\'e}& \multicolumn{1}{c|}{Slog}& \multicolumn{1}{c}{Souffl\'e}
\\
 \midrule 
 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{3-$k$-CFA}}}
 & 8 & 1,193 & 98.1k & 23.4k & 00:01 & 01:07 & 0:02 & 00:15 
&
 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{10-$m$-CFA}}}
 & 50 & 6,120 & 21k & 656k & 00:02  & 00:02 & 00:10 & 00:01
\\
 & 9 & 1,312 & 371k & 79.8k & 00:02 & 14:47 & 0:03 & 02:56 &
 & 100 & 11,670 & 42k & 2.78M & 00:07 & 00:09 & 00:20 & 00:04 
 \\
 & 10 & 1,431 & 1.44M & 291k & 00:06 & \timeout{} & 0:05 & 45:49 &
 & 200 & 22,770 & 86.5k & 11.4M & 00:26 & 00:56 &  00:42 & 00:23
\\
 & 11 & 1,550 & 5.68M &  1.11M & 00:27 & \timeout{} & 0:16 & \timeout{} & 
 & 400 & 44,970 & 173k & 46.4M  & 01:44 & 06:26 & 01:38 & 01:56 
\\ 
 & 12 & 1,669 & 22.5M & 4.32M & 02:14 & \timeout{} & 1:07 & \timeout{} &
 & 800 & 89,370 & 348k & 187M & 07:35 & 45:22 &  04:21 & 09:33
\\
 & 13 & 1,788 & 89.8M & 17.0M & 12:17 & \timeout{} & 5:08 & \timeout{} &
 & 1600 & 178,170 & 698k & 750M & 32:56 & \timeout{} & 14:36 & 1:02:35
 \\

 \midrule 
 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{4-$k$-CFA}}}
 & 9 & 1,363 & 312k & 65k & 00:01 & 14:38 & 00:03 & 02:08
&
 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{12-$m$-CFA}}}
 & 25  & 3,559  & 17k  & 385k    & 00:01 & $<$ \!\!\!\! :01 & 0:06 & $<$ \!\!\!\! :01  \\

 & 10 & 1,482 & 1.2M & 229k & 00:05 & \timeout{} & 00:05 & 40:30 &
 & 50  & 6,434  & 36k  & 1.89M  & 00:04 &00:03 &  0:11 & 00:03 \\

 & 11 & 1,601 & 4.69M & 853k & 00:20 & \timeout{} & 00:13 & \timeout{} &
 & 100 & 12,184 & 74k  & 8.82M  & 00:16 & 00:24 & 0:23 & 00:10 \\

 & 12 & 1,720 & 18.5M & 3.28M & 01:40 & \timeout{} & 00:53 & \timeout{} &
 & 200 & 23,684 & 151k & 34.6M & 01:10 & 02:37 & 0:53 & 00:55 \\

 & 13 & 1,839 & 73.8M & 12.9M & 08:44 & \timeout{} & 03:58 & \timeout{} &
 & 400 & 46,684 & 305k & 142M & 05:04 & 18:39 & 2:23 & 04:12 \\

 & 14 & 1,958 & 294M & 50.8M & 60:53 & \timeout{} & 35:46 & \timeout{} &
 & 800 & 92,684 & 611k  & 574M & 22:46 & 2:38:22 & 7:28 & 24:58 \\
 \midrule 

 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{5-$k$-CFA}}}
 & 9 & 1,429 & 203k & 50.7k & 00:02 & 05:30 & 0:03 & 01:15
&
 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{15-$m$-CFA}}}
 & 12  & 2,211  & 14.4k  & 137k &  00:01 & $<$ \!\!\!\! :01  & 0:04 & $<$ \!\!\!\! :01 
\\
 & 10 & 1,548 & 757k & 167k & 00:04 & 65:20 & 0:04 & 015:08  &
 & 24  & 3,591  & 35.9k  & 1.44M   &  00:03 & 00:02 & 0:06 & 00:01 
 \\
 & 11 & 1,667 & 2.91M  & 597k & 00:13 & \timeout{} &  0:08 & 196:06 &
 & 48  & 6,351  & 78.6k  & 8.29M   &  00:14 & 00:15 & 0:14 &  00:07
\\
 & 12 & 1,786 & 11.4M & 2.24M & 00:56 &  \timeout{}& 0:27 & \timeout{} &
  & 96  & 11,871 & 164k & 38.9M  &  01:08 & 01:41 & 0:36 & 00:36 
\\ 
 & 13 & 1,905 & 45.2M & 8.69M & 04:38 &  \timeout{}& 2:00 & \timeout{} &
 & 192 & 22,911 & 335k & 168M &  05:15 & 12:10 & 1:49 & 02:51 
\\
 & 14 & 2,024 & 180M & 34.2M & 25:14 & \timeout{}& 9:58 & \timeout{} &
 & 384 & 44,991 & 678k & 697M & 24:10 & 1:32:35 & 6:45 & 16:30 
 \\
 \bottomrule
 \end{tabular}
 \end{table*}


==> sec-apps-eqsat.tex <==
\subsection{Equality Saturation}
\label{sec:apps:eqsat}



==> sec-future.tex <==
\section{Future Work}
\label{sec:future}
%
...





==> sec-outro.tex <==
\section{Conclusion}
\label{sec:outro}
%
...




